Visual Drift Detection for Sequence Data Analysis of Business Processes

Event sequence data is increasingly available in various application domains, such as business process management, software engineering, or medical pathways. Processes in these domains are typically represented as process diagrams or flow charts. So far, various techniques have been developed for automatically generating such diagrams from event sequence data. An open challenge is the visual analysis of drift phenomena when processes change over time. In this paper, we address this research gap. Our contribution is a system for fine-granular process drift detection and corresponding visualizations for event logs of executed business processes. We evaluated our system both on synthetic and real-world data. On synthetic logs, we achieved an average F-score of 0.96 and outperformed all the state-of-the-art methods. On real-world logs, we identified all types of process drifts in a comprehensive manner. Finally, we conducted a user study highlighting that our visualizations are easy to use and useful as perceived by process mining experts. In this way, our work contributes to research on process mining, event sequence analysis, and visualization of temporal data.

==> addon/macros-DECLARE-drawing.tex <==
% for file in *.tex; do echo ${file%.*} | sed -e 's/^\(.\)/Draw\u\1/' | sed -e 's/\(.*\)/\\NewDocumentCommand{\\1}{ O{\$\\paramx\$} O{\$\\paramy\$} }{%/'; more "$file" | sed -e 's/\$\\paramx\$/#1/' | sed -e 's/\$\\paramy\$/#2/'; echo '%'; echo '}'; echo;  done > ../draw-Declare-macros.tex
\RequirePackage{xparse}

\NewDocumentCommand{\DrawAbsence}{ +O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..m$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltprec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltresp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.succ] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAtmostone}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..1$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnprec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnresp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.succ] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawCoex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.coex] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawEnd}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=End]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawExistence}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$n..\ast$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawInit}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=Init]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotchnsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.succ,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotcoex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.coex,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.succ,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawParticipation}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$1..\ast$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawPrec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawResex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.resex] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawResp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawSucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.succ] node {} (2);
\end{tikzpicture}%
}

==> addon/macros-DECLARE.tex <==
% \def\LTLFOfrag {\ensuremath{ \prescript{\land}{\circledast}{\forall\LTLf}} }
\def\LTLFOfrag {\ensuremath{\mathcal{L}_{\LTLf}^{\forall \wedge \circledast}}}

%\def\NowCns {\ensuremath{ \prescript{\vartimes\hspace{-1.25ex}\scalebox{0.75}{\lglobally}}{}{\Cns}}}
\def\CnsQu {\ensuremath{\Cns^{\text{q}}}}

\def\ActvSym {\ensuremath{\bullet}}
\def\Actv {\ensuremath{\varPhi_{\ActvSym}}}
\def\Trgt {\ensuremath{\varPhi_\Rightarrow}}
\def\Asgn {\ensuremath{\mathscr{A}}}
\def\Intrp {\ensuremath{\mathscr{I}}}
\def\IntrpA {\ensuremath{\Intrp_{\ActvSym}}}
\def\IntrpT {\ensuremath{\Intrp_\Rightarrow}}
\def\PreCns {\ensuremath{\prescript{\forall}{\Intrp}{\CnsTmp}}}
\def\PreCnsPrime {\ensuremath{\prescript{\forall}{\Intrp'}{\CnsTmp}}}

\def\NowCns {\ensuremath{\Cns^{(\ActvSym)}}}

\RequirePackage{xparse}
\NewDocumentCommand{\ActvC}{o}{%
  \ensuremath{\varphi_\bullet%
    \IfValueT{#1}{(#1)}%
  }%
}
\NewDocumentCommand{\CorrC}{o}{%
  \ensuremath{\varphi_\rightleftharpoons%
    \IfValueT{#1}{(#1)}%
  }%
}
\NewDocumentCommand{\TrgtC}{o}{%
  \ensuremath{\varphi_\Rightarrow%
    \IfValueT{#1}{(#1)}%
  }%
}

\NewDocumentCommand{\DeQuery}{m o}{%
\ensuremath{%
	\left\lbrack%
	#1 | \,%
	\IfValueTF{#2}{%
		#2%
	}{%
		(\CnsQu,\SuppMin,\ConfMin)
	}%
	\right\rbrack
}%
}

\def\ActvLang {\ensuremath{\mathscr{L}_\bullet}}
\def\TrgtLang {\ensuremath{\mathscr{L}_\Rightarrow}}

==> addon/macros-for-requirements-list.tex <==
%
% This one allows us to have a custom DESCRIPTION environment, in which numbers are preceded by a one-letter prefix.
% A short description can be added as an additional parameter to the begin-environment command.
% Successive references will have that very one-letter prefix + number with hyper-reference to it.
%
\RequirePackage{enumitem}
%
\def\requiprefix{R}
%
\newcounter{requicount}
\newlist{requidescr}{description}{1}
\setlist[requidescr,1]{%
	before={\setcounter{requicount}{0}%
		\renewcommand*\therequicount{\arabic{requicount}}},
	,font=\bfseries{\requiprefix}\stepcounter{requicount}\therequicount\normalfont.~\bfseries
}
%
% From https://tex.stackexchange.com/questions/1230/reference-name-of-description-list-item-in-latex
\makeatletter
\def\namedlabel#1{\begingroup
	\def\@currentlabel{\requiprefix\therequicount}%
	\phantomsection\label{#1}\endgroup
}
\makeatother
%
% Usage example:
% \begin{requidescr} % CUSTOM from CDC, with love
%   \item[\namedlabel{req:xaxis} Cluster on Y axis] Something more about that here.
% \end{requidescr}
% I especially like \ref{req:xaxis}.

==> addon/memorandum.tex <==
% !TeX root = ../main.tex
%
\section*{For us authors: some tips and tricks}
\label{sec:memo}
%%%
%%% Start of: preliminary commands to be used exclusively in this file.
%%%
\newglossaryentry{test}{name={test},description={A fictionary test}}
\newacronym{testacro}{TA}{Test Acronym}
%%%
%%% End of: preliminary commands to be used exclusively in this file.
%%%
%
% --------------------------------
% About comments
% --------------------------------
%
\hl{For your comments}, please use the
\todo[inline]{\texttt{todo} environment, either in-line or }
or aside.
\todo{aside}
%
You can even add missing figures with the \verb|\missingfigure| command (see \cref{fig:example:missing:figure}).
\begin{figure}[b]
\missingfigure{\texttt{{\textbackslash}missingfigure} command}
\caption{A missing figure}
\label{fig:example:missing:figure}
\end{figure}
%
\\
%
% --------------------------------
% About inline lists
% --------------------------------
%
\hl{For lowercase-roman-enumerated inline lists}, please use
\begin{iiilist}
\item the
\item \texttt{iiilist}
\item environment.
\end{iiilist}
It is a custom command you find in \verb|addons/commands.tex|. It is based on the \verb|\inparaenum| command, from package \textit{paralist}.
%
\\
%
% --------------------------------
% About keywords
% --------------------------------
%
\hl{For specific terms}, which may change in the future, add a \hl{glossary} entry in \texttt{addons/glossary.tex},
and use
\begin{iiilist}
\item the \texttt{gls} command to use them (e.g., \gls{test}),
\item the \texttt{Gls} command for capitalising them (e.g., \Gls{test}),
\item the \texttt{glspl} command for obtaining their plural form (e.g., \glspl{test}), and
\item the \texttt{Glspl} command for for obtaining their plural capitalised form (e.g., \Glspl{test}).
\end{iiilist}
It turns out to be very useful in those situations in which the co-authors do not remember, for example, whether they should indicate the sequences of executed actions as ``traces'' or ``runs''. To solve the issue and avoid that all co-authors write different things, they can decide on a temporary solution (say, ``traces''), make it a glossary entry (say, \verb+\newglossaryentry{actx}{name={trace},description={...}}+), use \verb+\gls{actx}+ (or similar commands -- see above) every time they want to say that thing, and when the opinion on the best term will change (in favour of ``runs''), it will be enough to change the glossary entry definition (\verb+\newglossaryentry{actxeq}{name={run},description={...}}+) and see it varied everywhere it was used in the text. Another use case is: ``AB Testing'' or ``AB testing''? To avoid that the ``T''s of ``testing'' occur as upper-case sometimes, and as lower-case at times, a single glossary entry comes handy!
%
\\
%
\hl{For acronyms}, they are meant be defined within the same file as follows: \texttt{{\textbackslash}newacronym\{testacro\}\{TA\}\{Test Acronym\}}.
They can be referenced by using \texttt{{\textbackslash}Gls} (plus variants for plural forms etc.).
Result is, you get the full version the first time the acronym is used
-- \texttt{{\textbackslash}gls\{testacro\}} is displayed as \Gls{testacro}.
From the second time onwards, the call will return the acronym only, without any description:
\texttt{{\textbackslash}gls\{testacro\}} is displayed as \Gls{testacro}.
To force the representation to have either long or short versions, use
\texttt{{\textbackslash}acrlong\{testacro\}}
(leading to \acrlong{testacro})
or
\texttt{{\textbackslash}acrshort\{testacro\}}
(displaying \acrshort{testacro}).
Acronyms are collected in \texttt{addons/glossary.tex} too.
%
\\
%
\hl{To refer to sections, tables, figures, etc.}, please use the \texttt{cref} command (e.g., \cref{sec:memo}).
\texttt{Cref} capitalises and expands the specifier of the referred document part (e.g., \Cref{fig:example:missing:figure}). It is best to be used at the beginning of phrases, whereas \texttt{cref} uses the abbreviation (e.g., \cref{fig:example:missing:figure}).

\begin{AuthNote}[CDC][Anything to add?]
	We can also add author's notes with the \verb|\begin{AuthNote}...\end{AuthNote}| environment. The optional parameters can be passed to the environment to add (1) your name tag or any in-line title, and (2) a side-note-like title.
\end{AuthNote}

==> addon/reduce-subsubsection-margin.tex <==
% https://tex.stackexchange.com/a/105577
%% Save the class definition of \subparagraph
\let\llncssubparagraph\subparagraph
%% Provide a definition to \subparagraph to keep titlesec happy
\let\subparagraph\paragraph
%% Load titlesec
\usepackage{titlesec}
%% Revert \subparagraph to the llncs definition
\let\subparagraph\llncssubparagraph
\titlespacing{\subsubsection}{0pt}{*0.5}{*0.5}


==> sections/visualization-change-esd.tex <==
%\todo[inline]{Here are TVCG papers and discussion}

%One important stream of the visualization research is a visualization of event sequence data~\cite{DBLP:series/hci/AignerMST11}. Some works accompany our research on the visualizations of drift behavior in temporal event sequence data. 
%\\
%The \emph{summarization of the event sequence data} for visual comprehension usually relies on the compound visual representations of different visualization types. The authors of \cite{DBLP:journals/tvcg/ChenXR18} use several connected views including the raw sequence representation and minimum description length principle-based. That shows the summary of the event sequence dat at a different granularity level. Another approach~\cite{DBLP:journals/tvcg/GuoXZGZC18} splits the event data into threads and stages. That allows summarizing before complex and long event sequences. The authors of~\cite{DBLP:journals/tvcg/ZhangCD19}  combine the raw event sequence visual representation with line plots containing additional measures attached. They also use several custom infographics to emphasize important use-case related characteristics. Other papers explain how to effectively visualize the \emph{alignment of event sequences}. The authors of ~\cite{DBLP:journals/tvcg/AlbersDG11} present the visual representation of the genome alignment that is structured by the hierachical relationships. Instead, the authors of~\cite{DBLP:journals/tvcg/CappersW18} visualize event sequences aligned by user-defined temporal rules. The visualizing change and \emph{drifts} in the event sequence data~\cite{DBLP:journals/tvcg/XuMR017} is achieved through compound views consisting of Marey’s graph, line plots, bar charts, calendar views, and custom infographics.





==> tables/table-example-log.tex <==
%!TEX root = ../main.tex
\renewcommand{\arraystretch}{1.6}
% Alternate row colours
\rowcolors{2}{white}{gray!12.5}
%\begin{tabular}{ l p{3cm} >{{\goodexample}~}l >{{\goodexample}~}l >{{\badexample}~}l c c}
\begin{tabular}{ l l l l l l }
	\toprule
	\textbf{Trace} & 
	\textbf{Activity 1} & 
	\textbf{Activity 2} & 
	\textbf{Activity 3} & 
	\textbf{Activity 4} & 
	\textbf{Activity 5} 
	\\
	\midrule
	
	$1$ & Lodging ticket &  Appeal & Appeal & Payment & Close ticket 
	\\
	$2$ & Lodging ticket &  Appeal & Appeal & No Payment & Close ticket 
	\\
	$3$ & Lodging ticket &  Appeal & Appeal & No Payment & Close ticket 
	\\
	$4$ & Lodging ticket  & Appeal & No Payment & Close ticket & Reopen ticket
	\\
	$5$ & Lodging ticket &  Appeal  & Payment & Close ticket &
	\\
	$6$ & Lodging ticket  & Appeal & No Payment & Close ticket &
	\\

	\bottomrule
\end{tabular}


==> tables/table-parameters.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l l l l l l}
	\toprule
	%\textbf{Approach}            &                                                                    \multicolumn{5}{c}{\textbf{Requirements}}                                                                    \\
	%\cmidrule{2-6}               & \textbf{R1}         & \textbf{R2}                                                                                             & \textbf{R3}         & \textbf{R4} & \textbf{R5} \\
	\textbf{Section}              & \textbf{Parameters} & \textbf{Description}                                                                                    & \textbf{Default}    &  \\ \midrule
	\ref{sec:declare:shift}       & \WinSize            & How many traces are used to calculate constraints in one step                                                       & Guideline provided  &  \\
	\ref{sec:declare:shift}       & \WinStep            & After each window is computed, how many traces we skip to move to calculating next window's                  & Guideline provided  &  \\
	\ref{sec:cluster-changepoint} & Cluster Algorithm   & We choose what method to use, to cluster traces into separate drifting groups             & Found optimal       &  \\
	                              & - Method            & Technique of how clustering algorithm calculates distance between clusters                   & Found optimal       &  \\
	                              & - Metric            & How the distance is calculated for two time-series                                                        & Found optimal       &  \\
	                              & - Criteria          & Criteria of cluster cut off                                                                             & Guideline 
provided &  \\
	                              & - Criteria Parameter & The cutoff value for \emph{Criteria} parameter                                                                     &                     &  \\
	\ref{sec:cluster-changepoint} & Sort Method Distance  & Distance metric to use for sorting inside of clusters & Found optimal       &  \\
	\ref{sec:cluster-changepoint} & Change Point Method   & The method to automatically detect drifts                                                               & Found optimal       &  \\
	                              & - CostFunction      & Cost function to calculate optimize cost point search                                                   & Found optimal       &  \\
	                              & - SearchMethod      & Change point search method                                                                              & Found optimal       &  \\ \bottomrule
\end{tabular} 
} 


==> tikzlibraryDECLARE.code.tex <==
%
% This is the DECLARE TikZ library by Claudio Di Ciccio is licensed under a Creative Commons Attribution-ShareAlike 4.0 International License.
% This work is licensed under the Creative Commons Attribution-ShareAlike 4.0 International License. To view a copy of this license, visit http://creativecommons.org/licenses/by-sa/4.0/.
%
% Author: Claudio Di Ciccio
% Website: www.diciccio.net
% Date: 2017/02/08
%
\usetikzlibrary{arrows.meta,decorations.markings}
\def\DTZU {2ex}
\tikzset{
 DECLARE.task/.style={
  rounded corners=1ex,
  minimum width=3em,
  minimum height=1ex,
  align=center,
  font=\sffamily,
  inner sep=5,
  draw
 },
 DECLARE.existcon/.style={
  label={[style=draw,yshift=-1\pgflinewidth]above:{\tiny \textit{#1}}}
 },
 DECLARE.neg/.style={
  semithick,
  postaction={decorate,decoration={markings,
   mark=at position .5 with {\arrow[xshift=0.15*\DTZU]{Bar[width=1.5*\DTZU]}},
   mark=at position .5 with {\arrow[xshift=-0.15*\DTZU]{Bar[width=1.5*\DTZU]}}
  }}
 },
 DECLARE.resex/.style={
  semithick,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-,
  shorten <=-0.5*\DTZU
 },
 DECLARE.resp/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU
 },
 DECLARE.alt.resp/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  double distance=0.25*\DTZU
 },
 DECLARE.chn.resp/.style={
  semithick,rounded corners,
  preaction={draw, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}
 },
 DECLARE.prec/.style={
  semithick,rounded corners,
  {-{Triangle[length=1*\DTZU,width=1*\DTZU]Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >=-0.5*\DTZU
 },
 DECLARE.alt.prec/.style={
  semithick,rounded corners,
  postaction={draw, shorten >= 0.5*\DTZU, double distance=0.25*\DTZU, {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.chn.prec/.style={
  semithick,rounded corners,
  preaction={draw, shorten >= 0.5*\DTZU, double distance=0.25*\DTZU, {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.succ/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]Circle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  shorten >=-0.5*\DTZU
 },
 DECLARE.coex/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Circle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  shorten >=-0.5*\DTZU
 },
 DECLARE.alt.succ/.style={
  semithick,rounded corners,
  postaction={draw, shorten >= 0.5*\DTZU, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.chn.succ/.style={
  semithick,rounded corners,
  preaction={draw, shorten >= 0.5*\DTZU, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 }
}
